Tight Revenue Gaps among Simple Mechanisms

We consider a fundamental problem in microeconomics: selling a single item to a number of potential buyers, whose values are drawn from known independent and regular (not necessarily identical) distributions. There are four widely-used and widely-studied mechanisms in the literature: {\sf Myerson Auction}~({\sf OPT}), {\sf Sequential Posted-Pricing}~({\sf SPM}), {\sf Second-Price Auction with Anonymous Reserve}~({\sf AR}), and {\sf Anonymous Pricing}~({\sf AP}). {\sf OPT} is revenue-optimal but complicated, which also experiences several issues in practice such as fairness; {\sf AP} is the simplest mechanism, but also generates the lowest revenue among these four mechanisms; {\sf SPM} and {\sf AR} are of intermediate complexity and revenue. We explore revenue gaps among these mechanisms, each of which is defined as the largest ratio between revenues from a pair of mechanisms. We establish two tight bounds and one improved bound: 1. {\sf SPM} vs.\ {\sf AP}: this ratio studies the power of discrimination in pricing schemes. We obtain the tight ratio of $\mathcal{C^*} \approx 2.62$, closing the gap between $\big[\frac{e}{e - 1}, e\big]$ left before. 2. {\sf AR} vs.\ {\sf AP}: this ratio measures the relative power of auction scheme vs.\ pricing scheme, when no discrimination is allowed. We attain the tight ratio of $\frac{\pi^2}{6} \approx 1.64$, closing the previously known bounds $\big[\frac{e}{e - 1}, e\big]$. 3. {\sf OPT} vs.\ {\sf AR}: this ratio quantifies the power of discrimination in auction schemes, and is previously known to be somewhere between $\big[2, e\big]$. The lower-bound of $2$ was conjectured to be tight by Hartline and Roughgarden (2009) and Alaei et al.\ (2015). We acquire a better lower-bound of $2.15$, and thus disprove this conjecture.

==> app_spm_ap_relaxations.tex <==
\paragraph{[Lemma~\ref{lem:spm_ap_relexation}].}
\emph{If Constraint~(\ref{cstr:spm_ap4}) is not tight for some $1 \leq k \leq n$, then there exists another triangular instance $\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n$ such that:
\begin{enumerate}
\item Respecting the new instance $\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n$, Constraint~(\ref{cstr:spm_ap4}) is tight for each $1 \leq k \leq n$;
\item The objective function of Program~\ref{prog:spm_ap1} increases.
\end{enumerate}}

\begin{proof}
We construct such $\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n$ by induction. Let $k$ be the smallest index for Constraint~(\ref{cstr:spm_ap4}) that is not tight, presented in the following:
\begin{align}
\label{eq:v_i}
& \sum\limits_{j = 1}^i \ln\left(1 + \frac{v_j q_j}{1 - q_j}\right) = \mathcal{R}(v_i) \quad\quad \forall 1 \leq i \leq k - 1 \\
\label{eq:v_k}
& \ln\left(1 + \frac{v_k q_k}{1 - q_k}\right) < \mathcal{R}(v_k) - \mathcal{R}(v_{k - 1})
\end{align}
We construct a new instance $\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n$ in the following way: for each $i \neq k$, let
\[
\label{eq:bar_v_i}
\overline{v}_i = v_i \quad\quad \overline{q}_i = q_i
\]
for k, define $\overline{v}_k$ and $\overline{q}_k$ that satisfy
\[
\label{eq:bar_v_k}
\ln\left(1 + \frac{\overline{v}_k \overline{q}_k}{1 - \overline{q}_k}\right) = \mathcal{R}(\overline{v}_k) - \mathcal{R}(v_{k - 1}) \quad\quad \overline{v}_k \overline{q}_k = v_k q_k.
\]

After such assignment, we claim that
\begin{itemize}
\item Such $\overline{v}_k$ and $\overline{q}_k$ certainly exist, and $v_k < \overline{v}_k < v_{k - 1}$ and $0 < \overline{q}_k < q_k$.
\item Respecting $\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n$, Constraint~(\ref{cstr:spm_ap4}) still holds for each $k + 1 \leq i \leq n$.
\end{itemize}

For the first claim, define $K(x) \eqdef \ln\left(1 + \frac{v_k q_k}{1 - \frac{v_k q_k}{x}}\right) - \mathcal{R}(x) + \mathcal{R}(v_{k - 1})$. Observe that
\[
\begin{aligned}
K(v_k) = \ln\left(1 + \frac{v_k q_k}{1 - q_k}\right) - \mathcal{R}(v_k) + \mathcal{R}(v_{k - 1}) \overset{(\ref{eq:v_k})}{<} 0 \quad\quad K(v_{k - 1}) = \ln\left(1 + \frac{v_k q_k}{1 - \frac{v_k q_k}{v_{k - 1}}}\right) > 0
\end{aligned}
\]
and $K(x)$ is continuous when $x \in [v_k, v_{k - 1}]$. According to the intermediate value theorem, there exists at least one $\overline{v}_k \in (v_k, v_{k - 1})$ such that $K(\overline{v}_k) = 0$ and $\overline{q}_k = \frac{v_k q_k}{\overline{v}_k} < q_k$. In addition, for each $k + 1 \leq i \leq n$,
\begin{flalign*}
& \sum\limits_{j = 1}^i \ln\left(1 + \frac{\overline{v}_j \overline{q}_j}{1 - \overline{q}_j}\right) \overset{(\ref{eq:bar_v_i})}{=} \sum\limits_{j = 1}^i \ln\left(1 + \frac{v_j q_j}{1 - q_j}\right) + \ln\left(1 + \frac{\overline{v}_k \overline{q}_k}{1 - \overline{q}_k}\right) - \ln\left(1 + \frac{v_k q_k}{1 - q_k}\right) \\
\overset{(\ref{cstr:spm_ap4})}{\leq} & \mathcal{R}(v_i) + \ln\left(1 + \frac{v_k q_k}{1 - \overline{q}_k}\right) - \ln\left(1 + \frac{v_k q_k}{1 - q_k}\right) < \mathcal{R}(v_i)
\end{flalign*}
where the last inequality is strict since $0 < \overline{q}_k < q_k$. This directly leads to our second claim.

Combining the above two claims together, for each $k + 1 \leq i \leq n$, we can construct desired $\overline{v}_i$ and $\overline{q}_i$ inductively. In summary,
\[
\label{eq:bar_vq}
\overline{v}_i \overline{q}_i = v_i q_i \quad\quad \overline{v}_i \geq v_i \quad\quad \overline{q}_i \leq q_i
\]
for each $1 \leq i \leq n$, where both inequalities are strict for each $k \leq i \leq n$. Eventually, the difference between $\spm\left(\{\tri(\overline{v}_i, \overline{q}_i)\}_{i = 1}^n\right)$ and $\spm\left(\{\tri(v_i, q_i)\}_{i = 1}^n\right)$ is
\[
1 + \sum\limits_{i = 1}^n \overline{v}_i \overline{q}_i \cdot \prod\limits_{j = 1}^{i - 1} (1 - \overline{q}_j) - 1 - \sum\limits_{i = 1}^n v_i q_i \cdot \prod\limits_{j = 1}^{i - 1} (1 - q_j) \overset{(\ref{eq:bar_vq})}{=} \sum\limits_{i = 1}^n v_i q_i \cdot \left[\prod\limits_{j = 1}^{i - 1} (1 - \overline{q}_j) - \prod\limits_{j = 1}^{i - 1} (1 - q_j)\right] > 0
\]
where the last inequality is strict since $\overline{q}_i < q_i$ for each $k \leq i \leq n$. This completes the proof of Lemma~\ref{lem:spm_ap_relexation}.
\end{proof}
